A Note on the Complexity of Model-Checking Bounded Multi-Pushdown Systems

In this note, we provide complexity characterizations of model checking multi-pushdown systems. Multi-pushdown systems model recursive concurrent programs in which any sequential process has a finite control. We consider three standard notions for boundedness: context boundedness, phase boundedness and stack ordering. The logical formalism is a linear-time temporal logic extending well-known logic CaRet but dedicated to multi-pushdown systems in which abstract operators (related to calls and returns) such as those for next-time and until are parameterized by stacks. We show that the problem is EXPTIME-complete for context-bounded runs and unary encoding of the number of context switches; we also prove that the problem is 2EXPTIME-complete for phase-bounded runs and unary encoding of the number of phase switches. In both cases, the value k is given as an input (whence it is not a constant of the model-checking problem), which makes a substantial difference in the complexity. In certain cases, our results improve previous complexity results.

==> section-usefulness.tex <==
\paragraph{Examples.}
\label{section-examples}
Our language allows us to talk about stack contents of multiple
threads, as well as talk about call and return behavior of multiple stacks.
%
For instance one may express notions such as atomicity:
certain operations (say proposition $p$ denotes that) are to be
operated consecutively on same stack before any other stack becomes active
$p \Rightarrow (\bigwedge_{s \in \mpsMoves} s \Rightarrow \next s)$;
or that of synchronization
barriers: that a certain state is reached in each thread
(say, denoted by proposition $p_s$ for stack $s$) before further progress is made:
$\bigwedge_{s \in \mpsMoves}(p_s \Rightarrow \neg s) \vee (\bigwedge_{s \in \mpsMoves} p_s)$. Important point to
notes is that the propositions $p_s$ can express thread-specific properties including
those of stack-contents using regularity constraints. Also, all properties about
about calls and returns, for instance X, Y, Z in [], can continue  to be asserted
because of our
introduction of $\next^a$/$\next^a_s$ and $\until^a$/$\until^a_s$ which is able to
isolate and reason about individual stacks.
%% 
%What about trying to express parallel assertions
%from~\cite{Schwartzetal12} or related works.



==> sync-figure-accept-cond.tex <==
\begin{figure}
\begin{enumerate}[(a)]
\item \label{buchi:until} % Until formulas
  $\forall \aformulabis = \aformula_1 \until \aformula_2 $:
  $F^1_{\aformulabis} = \inbrace{(\hat{\mpsState},\mpsMove) \ |
     \ \aformula_2 \in \atom_\mpsMove \vee 
     \aformulabis \notin \atom_\mpsMove}$
\item \label{buchi:absuntil} % Abstract-until formulas
  $\forall \aformulabis = \aformula_1 \until^\opAbs_j \aformula_2$:
  $F^2_{\aformulabis} = \inbrace{(\hat{\mpsState},\mpsMove) \ |
  \ j=\mpsMove, r_\mpsMove = \tNoRet, (\aformula_2 \in \atom_\mpsMove
  \text{ or } \aformulabis \notin \atom_\mpsMove) }$
\item \label{buchi:dead} % Dead tag
  $\forall j \in \mpsMoves$: 
  $ F^3_j = \inbrace{(\hat{\mpsState},\mpsMove) \ |\ j=\mpsMove } 
       \cup \inbrace{(\hat{\mpsState},\mpsMove) \ |\ \adtag_j = \tDead} $
\item \label{buchi:return} % Inf tag
  $\forall j \in \mpsMoves:$
  $ F^4_j = \inbrace{(\hat{\mpsState},\mpsMove) \ |\ \adtag_j = \tDead} \cup
            \inbrace{(\hat{\mpsState},\mpsMove) \ |\ j=\mpsMove, \adtag_\mpsMove = \tNoRet}
  $
\end{enumerate}
\caption{%
  Acceptance sets, subsets of $\hat{\mpsStates} \times \mpsMoves$.
  Notation, $\hat{\mpsState}=(\mpsState, \set{\atom_i}_i, \set{\artag_i}, \set{\adtag_i}_i) $
}\label{figure:acceptCond}
\end{figure}


==> sync-old-accept-cond.tex <==
The (B\"uchi) acceptance conditions are given by the following
sets. We use $\mpsState'$ as short-hand for $\inparen{\mpsState,
  \mpsMove, \{\atom_i\}, \{\artag_i\}, \{\adtag_i\}}$ in defining
subsets $\mpsStates'$
\begin{itemize}
\item % Until formulas
  For each until formula, $\aformulabis =
  \aformula_1 \until \aformula_2 $, define the set 
  \[F^1_{\aformulabis} = \inbrace{\mpsState' \in \mpsStates'\ |\ \aformula_2 \in \atom_\mpsMove \vee \aformulabis \notin \atom_\mpsMove }\]
\item % Abstract-until formulas
  For each abstract-until formula, $\aformulabis = \aformula_1
  \until^\opAbs_j \aformula_2$, define the set
  \[F^2_{\aformulabis} = \inbrace{\mpsState' \in \mpsStates'\ |\ j=\mpsMove, r_\mpsMove = \tNoRet, (\aformula_2 \in \atom_\mpsMove \text{ or } \aformulabis \notin \atom_\mpsMove) } \]
\item % Dead tag
  For each $j \in \mpsMoves$, define the set
  \[ F^3_j = \inbrace{\mpsState' \in \mpsStates'\ |\ j=\mpsMove } \cup 
             \inbrace{\mpsState' \in \mpsStates'\ |\ \adtag_j = \tDead}
  \]
  % Explanation:
  %% Dead tag is guessed correctly: Either the thread is "active"
  %% infinitely often, or the dead tag occurs infinitely often.
  %% \forall i. {(g,i,.....) } \cup
  %%            {(g,......,b_i,...) | b_i = dead}
  %% (If thread i is active only finite number of times, we will
  %%  hit a state such that b_i is dead. Since tags change only
  %%  when thread is active, it actually switches at the "correct"
  %%  time.)
\item % Inf tag
  For each $j \in \mpsMoves$, define the set
  \[ F^4_j = \inbrace{\mpsState' \in \mpsStates'\ |\ \adtag_j = \tDead} \cup
             \inbrace{\mpsState' \in \mpsStates'\ |\ j=\mpsMove, \adtag_\mpsMove = \tNoRet}
  \]
  % Explanation:
  %% Inf/noreturn tag is guessed correctly: If the thread does
  %% not become dead (is active infinitely often), the thread
  %% should have int/noreturn-tag infinitely often. (this was
  %% Buchi in the original paper -- i.e. when the notions of
  %% threads is removed)
  %% \forall i. {(g,...,) | b_i = dead} \cup
  %%            {(g,i,...,r_i) | r_i = inf}
\end{itemize}

Then the final acceptance conditions are just the set of above sets,
$F^1_\aformulabis$ over all until-formulas, $F^2_\aformulabis$ over
all abstract-until formulas, $F^3_j$ and $F^4_j$ for all $j \in
\mpsMoves$.


==> sync-old-trans-reln.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% transition relns --- now transformed into a figure -- added here mar 9 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





New Transition Relation
\[
 \mpsTrans_\mpsMove' : 
  \inparen{G \times \Atoms(\phi)^\mpsStackCount \times \tagsRet^\mpsStackCount \times \tagsDead^\mpsStackCount} \times
  \inparen{\mpsAlphabet \times \Atoms(\phi)}
  \to
\]
\[
  \inparen{G \times \Atoms(\phi)^\mpsStackCount \times \tagsRet^\mpsStackCount \times \tagsDead^\mpsStackCount} 
  \times \mpsMoves \times \actions'
%  \inparen{\actions \times \inparen{\mpsAlphabet \times \Atoms(\phi)} }
\]
\[ 
\delimitershortfall=-1pt
 \pair{
   \pair{\inparen{\mpsState, \{\atom_i\},\{\artag_i\},\{\adtag_i\}}}{(\mpsChar_S,\mpsChar_A)}
  }{
   \inparen{\inparen{\mpsState', \{\atom_i'\},\{\artag_i'\},\{\adtag_i'\}},\mpsMove',\anaction(\mpsChar_S',\mpsChar_A')}
 } \in \mpsTrans_\mpsMove'
\]
if
\begin{itemize}
\item Move in the original system: $\pair{(\mpsState,
  \mpsChar_S)}{(\mpsState', \mpsMove', \anaction(\mpsChar_S') )} \in
  \mpsTrans_\mpsMove$ \ref{trans:origTrans}
\item $\atom_\mpsMove$ and $\mpsState$ and $\mpsMove$ are
  \emph{consistent} with each other, that is $(g,s) \in
  \atom_\mpsMove$. \ref{trans:stateConsistent}
\item $\atom'_{s'}$ and $\mpsState'$ and $\mpsMove'$ consistent with
  each other. \ref{trans:newStateConsistent}
\item Tag and atom corresponding to only the current thread change: for
  all $j \neq \mpsMove$, $\atom_j = \atom_j'$, $\artag_j =
  \artag_j'$ and $\adtag_j = \adtag_j'$. \ref{trans:nochange}
\item Global Next.  $\next \atom_\mpsMove \subseteq
  \atom_{\mpsMove'}'$ ($=\atom_{\mpsMove'}$) where $\next A$ is
  defined to next formulas in $A$, $\inbrace{ \aformula \ |\ \next
    \aformula \in A}$. \ref{trans:globalnext}
% \item (*) Caller-next and Abstract-next formulas corresponding to only
%   current thread change: for all $j \neq \mpsMove$,
%   $\next^o_j \atom_{\mpsMove'}' = \next^o_j \atom_\mpsMove$
%   for $o \in \{\opAbs,\opCall\}$.
\item Dead tag.
  \begin{itemize} 
  %% \item No rising of the dead: $\adtag_j = \tDead$ implies
  %%   $\adtag_j' = \tDead$. % not required -- implied by earlier condition
  \item No ghosts: $\adtag_\mpsMove = \tAlive$. \ref{trans:activealive}
  \item Dying thread should have no abstract-next formulas to satisfy.
    $\adtag_\mpsMove' = \tDead$ implies $\next^\opAbs_\mpsMove
    \atom_\mpsMove = \emptyset$ \ref{trans:dyingObligFree}
  \end{itemize}
\item Push ($\anaction = \actCall$) 
  \begin{itemize}
  \item Stack atom. Push the current atom in the stack:
    $\mpsChar_A' = \atom_\mpsMove$. \ref{trans:pushStackAtom}
  \item Abstract next. Taken care by pushing on to stack, but
    shouldn't have any if we are never going to return:
    $\artag_\mpsMove = \tNoRet \implies \next^\opAbs_\mpsMove 
    \atom_\mpsMove = \emptyset$. \ref{trans:noreturnObligFree}
  \item (*) Caller next. Add caller formulas to all formulas possible:
    $\next^\opCall_\mpsMove \atom_{\mpsMove'}' =
    \next^\opCall_\mpsMove \Atoms(\aformula)
    \cap \atom_\mpsMove$ \ref{trans:pushHandleCaller}
  \item Return tag. This layer finite if previous one was:
    $\artag_\mpsMove = \tRet \implies \artag_\mpsMove' = \tRet$.
    \ref{trans:retTag1}
  \end{itemize}
\item Internal ($\anaction = \actInt$) 
  \begin{itemize}
  \item Abstract next, sent to next move of this thread:
    $\next^\opAbs_\mpsMove \atom_\mpsMove \subseteq \atom_\mpsMove'$.
    \ref{trans:internalHandleAbstract}
  \item Stack atom, caller next formulas and return tag stay same: $\mpsChar_A' = \mpsChar_A$,
  %\item Caller next, stay same:
    $\next^\opCall_\mpsMove
    \atom_{\mpsMove'}' = \next^\opCall_\mpsMove \atom_\mpsMove$,
  %\item Don't-return tag, stays same:
    $\artag_\mpsMove' = \artag_\mpsMove$. \ref{trans:internalUnchanged}
  \end{itemize}
\item Pop ($\anaction = \actRet$) 
  \begin{itemize}
  \item Stack atom. Handle the abstract next formulas:
    $\next^\opAbs_\mpsMove \mpsChar_A \subseteq \atom_\mpsMove'$.
    \ref{trans:returnStackAtom}
  \item Abstract next. Should not have any: $\next^\opAbs_\mpsMove
    \atom_\mpsMove = \emptyset$. \ref{trans:returnHandleAbstract}
  \item Caller next. Probably nothing to do here. \emph{not convinced
      though}
  \item Return tag. Be consistent, $\artag_\mpsMove = \tRet$ \ref{trans:retTag2}
  \end{itemize}
\end{itemize}


